Training Energy-Based Normalizing Flow with Score-Matching Objectives

In this paper, we establish a connection between the parameterization of flow-based and energy-based generative models, and present a new flow-based modeling approach called energy-based normalizing flow (EBFlow). We demonstrate that by optimizing EBFlow with score-matching objectives, the computation of Jacobian determinants for linear transformations can be entirely bypassed. This feature enables the use of arbitrary linear layers in the construction of flow-based models without increasing the computational time complexity of each training iteration from $O(D^2L)$ to $O(D^3L)$ for an $L$-layered model that accepts $D$-dimensional inputs. This makes the training of EBFlow more efficient than the commonly-adopted maximum likelihood training method. In addition to the reduction in runtime, we enhance the training stability and empirical performance of EBFlow through a number of techniques developed based on our analysis of the score-matching methods. The experimental results demonstrate that our approach achieves a significant speedup compared to maximum likelihood estimation while outperforming prior methods with a noticeable margin in terms of negative log-likelihood (NLL).

==> Equations/normalizing_constant.tex <==
\begin{equation}
\begin{aligned}
\bigg(\prod_{g_i\in \Sl}&\abs{\det (\jacob_{g_i}(\param))} \bigg)^{-1} \\
    &= \int_{\vx\in \Rd} \prior \of{g(\vx;\theta)}\prod_{g_i\in \Sn}\abs{\det (\jacob_{g_i}(\vx\,;\param))} d\vx.
\end{aligned}
    \label{eq:normalizing_constant}
\end{equation}
